Isthmus: Bridging Supervision Islands Restores Uncertainty and Stability in One-Step Flows

One-step flow maps are increasingly used as posterior samplers, where the point of sampling is the uncertainty that the samples carry. We find that the one-step sampler loses this uncertainty and becomes less stable. Compared with multi-step samples of the same network, its samples lose variance and decorrelate. Supervising the one-step jump directly makes this worse; the samples collapse further toward the conditional mean and break down when training is extended. We trace both failures to the locations where training places its pairs of start and end times. Only pairs on the diagonal of the time triangle receive targets from data, and the pair used for one-step sampling is either left unsupervised or supervised on an island, a set of pairs that the self-consistency identity does not connect to the diagonal, where the objective neither determines the one-step map nor anchors its training. We bridge the island with an isthmus, which places 5% of the training pairs along the whole edge of the triangle that joins the one-step pair to the diagonal. The error of the one-step map is then bounded by the self-consistency residual along this edge. With the network, the loss and the inference code unchanged and at no added cost, the isthmus improves one-step sampling across several flow-map objectives, in MRI reconstruction, face inpainting, and unconditional generation on CIFAR-10 and ImageNet 32x32. On brain MRI, it restores one-step calibration to 0.96 and the correlation with multi-step samples to 0.93; both vary far less across seeds, and the agreement holds when training is extended to three times its length.

==> supp_labels.tex <==
\makeatletter
\WarningFilter{hyperref}{Suppressing link with empty target}
\@namedef{r@S-cor:stability}{{S1}{6}{}{}{}}
\@namedef{r@S-cor:stability@cref}{{[spcorollary][1][]S1}{[1][6][]6}{}{}{}}
\@namedef{r@S-fig:direction}{{S10}{26}{}{}{}}
\@namedef{r@S-fig:direction@cref}{{[figure][10][]S10}{[1][25][]26}{}{}{}}
\@namedef{r@S-fig:heat}{{S8}{24}{}{}{}}
\@namedef{r@S-fig:heat@cref}{{[figure][8][]S8}{[1][22][]24}{}{}{}}
\@namedef{r@S-fig:mech-full}{{S5}{22}{}{}{}}
\@namedef{r@S-fig:mech-full@cref}{{[figure][5][]S5}{[1][21][]22}{}{}{}}
\@namedef{r@S-fig:share}{{S9}{24}{}{}{}}
\@namedef{r@S-fig:share@cref}{{[figure][9][]S9}{[1][24][]24}{}{}{}}
\@namedef{r@S-lem:fixedpoint}{{S1}{4}{}{}{}}
\@namedef{r@S-lem:fixedpoint@cref}{{[splemma][1][]S1}{[1][4][]4}{}{}{}}
\@namedef{r@S-prop:band}{{S3}{7}{}{}{}}
\@namedef{r@S-prop:band@cref}{{[spproposition][3][]S3}{[1][7][]7}{}{}{}}
\@namedef{r@S-prop:dyn}{{S5}{11}{}{}{}}
\@namedef{r@S-prop:dyn@cref}{{[spproposition][5][]S5}{[1][11][]11}{}{}{}}
\@namedef{r@S-prop:exact}{{S1}{5}{}{}{}}
\@namedef{r@S-prop:exact@cref}{{[spproposition][1][]S1}{[1][5][]5}{}{}{}}
\@namedef{r@S-prop:ident}{{S4}{8}{}{}{}}
\@namedef{r@S-prop:ident@cref}{{[spproposition][4][]S4}{[1][8][]8}{}{}{}}
\@namedef{r@S-prop:value}{{S2}{7}{}{}{}}
\@namedef{r@S-prop:value@cref}{{[spproposition][2][]S2}{[1][7][]7}{}{}{}}
\@namedef{r@S-rem:td}{{S1}{12}{}{}{}}
\@namedef{r@S-rem:td@cref}{{[remark][1][]S1}{[1][12][]12}{}{}{}}
\@namedef{r@S-sec:conventions}{{S1}{3}{}{}{}}
\@namedef{r@S-sec:conventions@cref}{{[section][1][]S1}{[1][3][]3}{}{}{}}
\@namedef{r@S-sec:distortion}{{S8}{19}{}{}{}}
\@namedef{r@S-sec:distortion@cref}{{[section][8][]S8}{[1][19][]19}{}{}{}}
\@namedef{r@S-sec:dyn}{{S11}{26}{}{}{}}
\@namedef{r@S-sec:dyn@cref}{{[section][11][]S11}{[1][26][]26}{}{}{}}
\@namedef{r@S-sec:eval}{{S7}{18}{}{}{}}
\@namedef{r@S-sec:eval@cref}{{[section][7][]S7}{[1][18][]18}{}{}{}}
\@namedef{r@S-sec:family}{{S5}{14}{}{}{}}
\@namedef{r@S-sec:family@cref}{{[section][5][]S5}{[1][14][]14}{}{}{}}
\@namedef{r@S-sec:impl}{{S6}{15}{}{}{}}
\@namedef{r@S-sec:impl@cref}{{[section][6][]S6}{[1][15][]15}{}{}{}}
\@namedef{r@S-sec:lg}{{S3}{13}{}{}{}}
\@namedef{r@S-sec:lg@cref}{{[section][3][]S3}{[1][13][]13}{}{}{}}
\@namedef{r@S-sec:mri}{{S9}{20}{}{}{}}
\@namedef{r@S-sec:mri@cref}{{[section][9][]S9}{[1][20][]20}{}{}{}}
\@namedef{r@S-sec:proofs}{{S2}{3}{}{}{}}
\@namedef{r@S-sec:proofs@cref}{{[section][2][]S2}{[1][3][]3}{}{}{}}
\@namedef{r@S-sec:related-ext}{{S14}{34}{}{}{}}
\@namedef{r@S-sec:related-ext@cref}{{[section][14][]S14}{[1][34][]34}{}{}{}}
\@namedef{r@S-tab:family}{{S2}{16}{}{}{}}
\@namedef{r@S-tab:family@cref}{{[table][2][]S2}{[1][15][]16}{}{}{}}
\@namedef{r@S-tab:fastmri}{{S16}{30}{}{}{}}
\@namedef{r@S-tab:fastmri@cref}{{[table][16][]S16}{[1][29][]30}{}{}{}}
\@namedef{r@S-tab:long}{{S12}{27}{}{}{}}
\@namedef{r@S-tab:long@cref}{{[table][12][]S12}{[1][27][]27}{}{}{}}
\@namedef{r@S-tab:mri-full}{{S7}{21}{}{}{}}
\@namedef{r@S-tab:mri-full@cref}{{[table][7][]S7}{[1][20][]21}{}{}{}}
\@namedef{r@S-tab:snap-ixi}{{S10}{25}{}{}{}}
\@namedef{r@S-tab:snap-ixi@cref}{{[table][10][]S10}{[1][25][]25}{}{}{}}
\@namedef{r@S-tab:uncond-seeds}{{S18}{30}{}{}{}}
\@namedef{r@S-tab:uncond-seeds@cref}{{[table][18][]S18}{[1][30][]30}{}{}{}}
\makeatother

